Frequency Limited $\mathcal{H}_2$ Optimal Model Reduction of Large-Scale Sparse Dynamical Systems

We mainly consider the frequency limited $\mathcal{H}_2$ optimal model order reduction of large-scale sparse generalized systems. For this purpose we need to solve two Sylvester equations. This paper proposes efficient algorithm to solve them efficiently. The ideas are also generalized to index-1 descriptor systems. Numerical experiments are carried out using Python Programming Language and the results are presented to demonstrate the approximation accuracy and computational efficiency of the proposed techniques.

==> csnameendcsname.tex <==
\relax 
\@setckpt{csnameendcsname\relax }{
\setcounter{page}{10}
\setcounter{equation}{16}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{1}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{5}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{1}
\setcounter{table}{1}
\setcounter{parentequation}{0}
\setcounter{caption@flags}{4}
\setcounter{continuedfloat}{0}
\setcounter{subfigure}{2}
\setcounter{subtable}{0}
\setcounter{ALC@unique}{0}
\setcounter{ALC@line}{0}
\setcounter{ALC@rem}{0}
\setcounter{ALC@depth}{0}
\setcounter{AlgoLine}{11}
\setcounter{algocfline}{3}
\setcounter{algocfproc}{3}
\setcounter{algocf}{3}
\setcounter{definition}{0}
\setcounter{conj}{0}
\setcounter{example}{3}
\setcounter{Maxaffil}{2}
\setcounter{authors}{4}
\setcounter{affil}{1}
}


==> preamble.tex <==
%\usepackage[hardware,software]{latexmacros/mymacros}
\usepackage{amsthm}
\usepackage{pgfplots}

\usepackage[vlined,longend,linesnumbered,ruled]{algorithm2e}
\providecommand{\dontprintsemicolon}{\DontPrintSemicolon}
\providecommand{\DontPrintSemicolon}{\dontprintsemicolon}
%\usepackage[colorlinks=true]{hyperref}

\usepackage[list=true]{caption,subcaption} %list=true enables listing
                                %of subfigures in the list of figures
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\usepackage{pgfplots}
\definecolor{mpiblue}{HTML}{006AA9}
\definecolor{mpigreen}{HTML}{5C871D}
\pgfplotscreateplotcyclelist{mylist1}{%
{black,solid},
{blue,dashed},
{mpigreen,dash pattern = on 3pt off 1pt on 1pt off 1pt},
{red,dash pattern = on 2pt off 2pt on 1pt off 2pt on 1pt off 2pt},
{cyan,densely dashed},
{mpiblue,densely dotted},
{magenta,dotted},
}
\pgfplotsset{every axis plot/.append style={line width=.75pt}}
%\DeclareMathOperator{\nul}{Null}
\DeclareMathOperator{\rang}{Rang}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rank}{rank}
\DeclareMathOperator{\eps}{eps}
%\DeclareMathOperator{\Rel}{Re}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\det}{de}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newcommand\norm[1]{\left\lVert#1\right\rVert}

% some help for emacs tex user
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main" 
%%% TeX-PDF-mode:t
%%% auto-fill-function:nil
%%% mode:auto-fill
%%% flyspell-mode:nil
%%% mode:flyspell
%%% ispell-local-dictionary: "en_US"
%%% End: 
     


